Prompting DirectSAM for Semantic Contour Extraction in Remote Sensing Images

The Direct Segment Anything Model (DirectSAM) excels in class-agnostic contour extraction. In this paper, we explore its use by applying it to optical remote sensing imagery, where semantic contour extraction-such as identifying buildings, road networks, and coastlines-holds significant practical value. Those applications are currently handled via training specialized small models separately on small datasets in each domain. We introduce a foundation model derived from DirectSAM, termed DirectSAM-RS, which not only inherits the strong segmentation capability acquired from natural images, but also benefits from a large-scale dataset we created for remote sensing semantic contour extraction. This dataset comprises over 34k image-text-contour triplets, making it at least 30 times larger than individual dataset. DirectSAM-RS integrates a prompter module: a text encoder and cross-attention layers attached to the DirectSAM architecture, which allows flexible conditioning on target class labels or referring expressions. We evaluate the DirectSAM-RS in both zero-shot and fine-tuning setting, and demonstrate that it achieves state-of-the-art performance across several downstream benchmarks.

==> figure/SLSD.tex <==
\begin{figure}[t]
\centering
% \hspace*{-0.42cm}
\includegraphics[width=1\columnwidth]{figure/SLSD.pdf}
\caption{\textbf{Inference result on SLSD}}
\label{fig:SLSD}
\end{figure}

==> figure/visual_feature.tex <==
\begin{figure}[ht]
\begin{center}
\includegraphics[width=0.9\columnwidth]{figure/visual_feature_p.pdf}
\caption{The visualization results of the first-level feature map \( \mathbf{F}_1 \) (left) and the second-level feature map \( \mathbf{F}_2 \) (right).}\label{fig:visual_feature}
\end{center}
\end{figure}

==> table/DG.tex <==



\begin{table}[t]
\centering
\caption{Road Extraction comparison on DeepGlobe dataset.}
\small
\label{tab:DeepGlobe}
\resizebox{\columnwidth}{!}{
\begin{tabular}{ccccccc}
\toprule
Method & ODS & OIS & F1 & LineIoU@3 & LineIoU@5 & AP \\ \hline
\rule{0pt}{2.2ex}
SwinT+OADecoder & 0.9389 & 0.6884 & 0.7531 & 0.1728 & 0.2379 & 0.8007 \\
DirectSAM-RS & 0.9190 & 0.6837 & 0.7506 & 0.1728 & 0.2379 & 0.7268 \\
DirectSAM-RS & 1 & 1 & 1 & 1 & 1 & 1 \\
DirectSAM-RS & 1 & 1 & 1 & 1 & 1 & 1 \\
 \bottomrule
\end{tabular}
}
\end{table}

==> table/DirectSAM-RS_pre_ablation.tex <==
% \begin{table}[]
% \centering

% \caption{\textbf{DirectSAM-RS LoveDA ablation study.} The metric used is the fixed contour threshold F1 score (ODS-F), and PT represents the pretrained weights.}
% \label{LD_ablation}
% \resizebox{\columnwidth}{!}{
% % \fontsize{9pt}{11pt}\selectfont
% \begin{tabular}{ccccccc}
% \toprule
%  & Agriculture & Barren & Building & Forest & Road & Water \\ \hline
%  \rule{0pt}{2.3ex}
% DirectSAM & 0.668 & 0.666 & 0.759 & 0.756 & 0.806 & 0.711 \\
% DirectSAM w/o PT & 0.625 & 0.606 & 0.654 & 0.673 & 0.757 & 0.639 \\
% \bottomrule
% \end{tabular}
% }
% \end{table}





\begin{table}[t]
\centering
\caption{\textbf{Training dataset ablation study on several tasks.} The metric used is the fixed contour threshold F1 score (ODS-F), and PT represents the pretrained weights.}
\label{DirectSAM-RS pre ablation}
\resizebox{\columnwidth}{!}{
\begin{tabular}{ccccc}
\toprule
Setting & LoveDA & DeepGlobe & BUBE & SLSD \\ \hline
\rule{0pt}{2.3ex}
DirectSAM-RS & 1 & 1 & 1 & 1 \\
DirectSAM-RS w/o PT & 1 & 1 & 1 & 1 \\
\bottomrule
\end{tabular}
}
\end{table}

==> table/GB.tex <==
% \begin{table}[htp]
%     \centering
%     \fontsize{9pt}{11pt}\selectfont
%     \caption{Edge Detection Accuracy of our model}
%     \label{table1}
%     \captionsetup[table]{skip=0pt}
%     % \begin{adjustbox}{width=0.72\linewidth} % 设置表格宽度
%         \begin{tabular}{lccc}
%             \toprule
%             Method & ODS-F & {\color[HTML]{000000} \begin{tabular}[c]{@{}c@{}}Line IoU\\ (Kernel=3)\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Line IoU\\ (Kernel=5)\end{tabular} \\
%             \midrule
%             BDCN & 0.5362 & 0.3233 & 0.3849 \\
%             SDLED & 0.8419 & 0.5089 & 0.6152 \\
%             Ours & \textbf{0.8504} & \textbf{0.5176} & \textbf{0.6378} \\ % 0.08 0.13
%             \bottomrule
%         \end{tabular}
%     % \end{adjustbox}
% \end{table}


\begin{table}[t]
\centering
\caption{Urban Building Contour Extraction on BUBE}
\label{tab:BUBE}
% \resizebox{\columnwidth}{!}{
% \fontsize{9pt}{11pt}\selectfont
\small
\begin{tabular}{cccc}
\toprule
Method & F1 & LineIou@3 & LineIou@5 \\ \hline
\rule{0pt}{2.2ex}
BDCN & 0.5362 & 0.3233 & 0.3849 \\
SDLED & 0.8419 & 0.5089 & 0.6152 \\
DirectSAM & \textbf{0.8504} & \textbf{0.5176} & \textbf{0.6378} \\
 \bottomrule
\end{tabular}
% }
\end{table}


% \begin{table}[htp]
% \centering
% \caption{Performance comparison on SLSD}
% \label{table3}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{ccccccc}
% \toprule
% Method & ODS & OIS & F1 & LineIoU@3 & LineIoU@5 & AP \\ \hline
% \rule{0pt}{2.2ex}
% HED & 0.8072 & 0.994 & 0.8973 & 0.5682 & 0.6267 & 0.9010 \\
% DirectSAM-RS & 0.8983 & 1 & 0.9278 & 0.6754 & 0.7267 & 0.9286 \\
% DirectSAM-RS &  & 1 &  &  &  &  \\
% DirectSAM-RS &  & 1 &  &  &  &  \\
%  \bottomrule
% \end{tabular}
% }
% \end{table}

==> table/GB1.tex <==


\begin{table}[]
\caption{Edge Detection Accuracy of our model}
\label{table1}
\begin{tabular}{cccc}
\hline
Method & ODS-F & {\color[HTML]{000000} Line IoU(Kernel=3)} & Line IoU(Kernel=5) \\ \hline
BDCN & 0.5362 & 0.3233 & 0.3849 \\
SDLED & 0.8419 & 0.5089 & 0.6152 \\
Ours & 0.8504 & 0.5176 & 0.6378 \\ \hline
\end{tabular}
\end{table}

==> table/LD_ablation_categories.tex <==
% \begin{table}[h]
% \centering
% \caption{Edge Detection Accuracy of our model}
% \label{table2}
% \resizebox{0.82\columnwidth}{!}{%
% \begin{tabular}{@{}ccc@{}}
% \toprule
% \multicolumn{1}{l}{} & DirectSAM & DirectSAM w/o pretraining \\ \midrule
% Barren & 0.666 & 0.606 \\
% Water & 0.711 & 0.639 \\
% Road & 0.806 & 0.757 \\
% Agriculture & 0.688 & 0.625 \\
% Forest & 0.756 & 0.673 \\
% Building & 0.759 & 0.654 \\ \bottomrule
% \end{tabular}%
% }
% \end{table}


\begin{table}[t]
\centering

\caption{\textbf{Pretrained weights ablation study for DirectSAM-RS.} The metric used is the ODS(Optimal Dataset Scale), and PT represents the pre-training weights.}
\label{SA1B_ablation_DR}
\resizebox{\columnwidth}{!}{
% \fontsize{9pt}{11pt}\selectfont
\begin{tabular}{ccccccc}
\toprule
 Setting& Agriculture & Barren & Building & Forest & Road & Water \\ \hline
 \rule{0pt}{2.3ex}
DirectSAM & 0.668 & 0.666 & 0.759 & 0.756 & 0.806 & 0.711 \\
DirectSAM w/o PT & 0.625 & 0.606 & 0.654 & 0.673 & 0.757 & 0.639 \\
\bottomrule
\end{tabular}
}
\end{table}



% \begin{table}[htp]
% \centering
% \caption{Performance comparison on SLSD}
% \label{table3}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{ccccccc}
% \toprule
% Method & ODS & OIS & F1 & LineIoU@3 & LineIoU@5 & AP \\ \hline
% \rule{0pt}{2.2ex}
% HED & 0.8072 & 0.994 & 0.8973 & 0.5682 & 0.6267 & 0.9010 \\
% DirectSAM-RS & 0.8983 & 1 & 0.9278 & 0.6754 & 0.7267 & 0.9286 \\
% DirectSAM-RS &  & 1 &  &  &  &  \\
% DirectSAM-RS &  & 1 &  &  &  &  \\
%  \bottomrule
% \end{tabular}
% }
% \end{table}

==> table/SLSD.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Coastline extraction benchmark on SLSD dataset.} }
\small
\label{tab:SLSD}
\resizebox{\columnwidth}{!}{

\begin{tabular}{ccccccc}
\toprule
Method & ODS & OIS & F1 & LineIoU@3 & LineIoU@5 & AP \\ \hline
\rule{0pt}{2.2ex}
HED & 0.8072 & 0.994 & 0.8973 & 0.6682 & 0.7267 & 0.9010 \\
DirectSAM-RS & 0.8983 & 1 & 0.9278 & 0.7754 & 0.8267 & 0.9286 \\
DirectSAM-RS &  & 1 &  &  &  &  \\
DirectSAM-RS &  & 1 &  &  &  &  \\
 \bottomrule
\end{tabular}
}

\end{table}




% \begin{table}[t]
% \centering
% \caption{\textbf{Coastline extraction benchmark on SLSD dataset.} }
% \small
% \label{tab:SLSD}
% % \resizebox{\columnwidth}{!}{
% \begin{tabularx}{\columnwidth}{cXXXXXX}
% \toprule
% Method & ODS & OIS & F1 & LineIoU@3 & LineIoU@5 & AP \\ \hline
% \rule{0pt}{2.2ex}
% HED & 0.8072 & 0.994 & 0.8973 & 0.5682 & 0.6267 & 0.9010 \\
% DirectSAM-RS & 0.8983 & 1 & 0.9278 & 0.6754 & 0.7267 & 0.9286 \\
% DirectSAM-RS &  & 1 &  &  &  &  \\
% DirectSAM-RS &  & 1 &  &  &  &  \\
%  \bottomrule
% \end{tabularx}
% % }

% \end{table}






% \begin{table}[h]
% \centering
% \caption{Edge Detection Accuracy of our model}
% \label{table2}
% \resizebox{0.82\columnwidth}{!}{%
% \begin{tabular}{@{}ccc@{}}
% \toprule
% \multicolumn{1}{l}{} & DirectSAM & DirectSAM w/o pretraining \\ \midrule
% Barren & 0.666 & 0.606 \\
% Water & 0.711 & 0.639 \\
% Road & 0.806 & 0.757 \\
% Agriculture & 0.688 & 0.625 \\
% Forest & 0.756 & 0.673 \\
% Building & 0.759 & 0.654 \\ \bottomrule
% \end{tabular}%
% }
% \end{table}

==> table/benchmark.tex <==


\begin{table}[t]

\centering
\caption{\textbf{Semantic Landmarks Contour Extraction.} Under the same training recipe as DirectSAM-RS, we reproduce the previous methods and evaluate them on the same validation set.}
\label{tab:SA1B_ablation_DRRS}
\resizebox{\columnwidth}{!}{
% \fontsize{9pt}{11pt}\selectfont
\small
\begin{tabular}{ccccccccc}
\toprule
Methods & ODS & OIS & LineIoU@3 & LineIoU@5 & AP \\ \hline
\rule{0pt}{2.2ex}
LSTM-CNN\cite{LSTMCNN} & 0.1552 & 0.5247 & 0.0795 & 0.0941 & 0.1231\\
% \rule{0pt}{1ex}
ConvLSTM\cite{ConvLSTM} & 0.2174 & 0.6485 & 0.1309 & 0.1544 & 0.1517 \\
LAVT\cite{lavt} & 0.2616 & 0.7859 & 0.2863 & 0.3449 & 0.5928\\
 RRSIS\cite{rrsis} & 0.2878 & 0.8143 & 0.3062 & 0.3754 & 0.6097\\
 DirectSAM-RS & 0.3684 & 0.8905 & 0.3586 & 0.4491 & 0.6314\\ 
 DirectSAM-RS w/o PT & 0.3251 & 0.8812 & 0.3251 & 0.4361 & 0.6172 \\
 \bottomrule
 \end{tabular}
}
\end{table}

==> table/zero_shot.tex <==



% \begin{table}[]
% \begin{tabular}{cccc}
% \hline
%  & LRSNY & SLSD & BUBE \\ \hline
% ODS &  &  &  \\ \hline
% \end{tabular}
% \end{table}

% \begin{table}[htp]
% \centering
% \caption{Zero-shot performance on DirectSAM-RS}
% \label{tab:zero-shot}
% % \resizebox{\columnwidth}{!}{
% % \fontsize{9pt}{11pt}\selectfont
% \small
% \begin{tabular}{cccc}
% \toprule
%  & LRSNY & SLSD & BUBE \\ \hline
% \rule{0pt}{2.4ex}
% ODS &  &  &  \\
%  \bottomrule
% \end{tabular}
% % }
% \end{table}

\begin{table}[htp]
\centering
\caption{Zero-shot performance on DirectSAM-RS}
\label{tab:zero-shot}
\resizebox{\columnwidth}{!}{
\small
\begin{tabular}{ccccccc}
\toprule
Dataset & ODS & OIS & F1 & LineIou@3 & LineIou@5 & AP \\ \hline
\rule{0pt}{2.3ex}
LRSNY & 0.3380 & 0.9105 & 0.6538 & 0.2438 & 0.3373 & 0.4642 \\
BUBE & 0.3738 & 0.8986 & 0.8212 & 0.3286 & 0.4373 & 0.6317 \\
SLSD & 0.1562 & 0.8025 & 0.6395 & 0.2163 & 0.3040 & 0.3560 \\ \hline
\end{tabular}
}
\end{table}



% \begin{table}[t]
% \centering
% \caption{\textbf{Zero-shot performance on DirectSAM-RS.} }
% \small
% \label{tab:zero-shot}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{ccccccc}
% \toprule
%  & LRSNY & SLSD & BUBE \\ \hline
% \rule{0pt}{2.2ex}
% ODS &  &  &  \\
%  \bottomrule
% \end{tabular}
% }
% \end{table}
